Computing Essential Sets for Convex and Non-convex Scenario Problems: Theory and Application

The scenario approach is a general data-driven algorithm to chance-constrained optimization. It seeks the optimal solution that is feasible to a carefully chosen number of scenarios. A crucial step in the scenario approach is to compute the cardinality of essential sets, which is the smallest subset of scenarios that determine the optimal solution. This paper addresses the challenge of efficiently identifying essential sets. For convex problems, we demonstrate that the sparsest dual solution of the scenario problem could pinpoint the essential set. For non-convex problems, we show that two simple algorithms return the essential set when the scenario problem is non-degenerate. Finally, we illustrate the theoretical results and computational algorithms on security-constrained unit commitment (SCUC) in power systems. In particular, case studies of chance-constrained SCUC are performed in the IEEE 118-bus system. Numerical results suggest that the scenario approach could be an attractive solution to practical power system applications.

==> main.tex <==

\section{Introduction}
\label{sec:introduction}
Security-constrained Unit commitment (SCUC) is one of the most important decisions made in power system operational planning. The SCUC problem seeks the most cost-efficient on/off decisions and dispatch schedules for generators, considering various security constraints such as generation and transmission capacity limits under contingencies.

SCUC is a decision making problem in uncertain environments by its nature.
Conventional SCUC problems ensure the system is secured for a number of outages in generation, transmission, or other elements within the system.
As the generation portfolio is shifting towards renewable resources, 
SCUC, a crucial part of power system day-ahead scheduling, needs to evolve to address the flexibility concerns.

\emph{Stochastic} optimization (SO) and \emph{robust} optimization (RO) are two common approaches for decision making under uncertainties. Both SO and RO have been successfully applied in various areas. SO relies on probabilistic models to depict uncertainties and often optimizes the objective function in the presence of randomness.
SO has found many successful applications in power system operations and planning problems.
For instance, references \cite{takriti_stochastic_1996,wu_stochastic_2007,zheng_stochastic_2015} formulate and solve the \emph{stochastic unit commitment} problem, which minimizes the expected commitment and dispatch costs. RO takes an alternative approach, in which the uncertainty model is set-based and typically deterministic \cite{bertsimas_theory_2011}. Recently, researchers in \cite{bertsimas_adaptive_2013} formulated and solved the \emph{robust unit commitment} problem, which minimizes the commitment and dispatch costs for the worst case in a predefined uncertainty set. 

This paper provides a perspective of solving SCUC in uncertain environments through the lens of chance-constrained optimization (CCO), which is akin to both SO and RO \cite{geng_data-driven_2019-2}. The main distinction between CCO and SO/RO is the \emph{chance constraint} (see \eqref{form:cc_opt_function_cc} and \eqref{form:cc_opt_cc} in Section \ref{sec:introduction_to_the_scenario_approach}), which explicitly considers the feasibility of solutions under uncertainties.
Various formulations of chance-constrained SCUC (c-SCUC) have been proposed, e.g., \cite{ozturk_solution_2004,pozo_chance-constrained_2013,wang_chance-constrained_2012,zhao_expected_2014,tan_hybrid_2016,bagheri_data-driven_2017,zhang_chance-constrained_2017-1,wang_price-based_2013,wu_chance-constrained_2014}. As mentioned in \cite{geng_data-driven_2019-2}, chance-constrained optimization problems can be solved using the scenario approach, sample average approximation, or robust optimization based techniques. We take c-SCUC as an example. It is solved via sample average approximation in \cite{wang_chance-constrained_2012,wang_price-based_2013,zhao_expected_2014,tan_hybrid_2016,bagheri_data-driven_2017,zhang_chance-constrained_2017-1,wu_chance-constrained_2014} and via robust optimization based techniques in \cite{jiang_robust_2012,margellos_stochastic_2013,hreinsson_stochastic_2015}\footnote{The method used in \cite{margellos_stochastic_2013,hreinsson_stochastic_2015} is based on \cite{margellos_road_2014}. It utilizes the sample complexity bound by an earlier version of the scenario approach \cite{alamo_sample_2010}, however, it is more closely related with robust optimization. Furthermore, the results in in \cite{margellos_stochastic_2013,hreinsson_stochastic_2015} might be overly conservative, since the sample complexity bound by \cite{alamo_sample_2010} could be significantly tightened by in-depth analysis of the scenario approach, see Theorem \ref{thm:exact_feasibility_scenario_approach} for more details.}.

\XG{References to be added \cite{ahmed_relaxations_2018} \cite{ahmed_solving_2008} \footnote{Nonanticipative duality, relaxations,
and formulations for chance-constrained stochastic programs, Convex relaxations of
chance constrained optimization problems} and \cite{bienstock_chance-constrained_2014} }

The scenario approach is a well-known algorithm to solve CCO problems \cite{calafiore_uncertain_2005,campi_exact_2008,calafiore_random_2010}. It was mainly targeted at convex problems (see Assumption \ref{ass:convexity}), whereas SCUC is non-convex by nature due to on/off commitment decisions. Consequently, the scenario approach was considered \emph{not applicable} for c-SCUC. An extended version of the scenario approach was proposed recently in \cite{campi_general_2018}, which makes it applicable for non-convex problems such as SCUC.

Our previous paper \cite{geng_chance-constrained_2019} might be the first attempt to apply the scenario approach on unit commitment\footnote{We call it unit commitment instead of SCUC because no security constraints are considered.}. However, the formulation therein is greatly simplified by ignoring some critical constraints such as transmission capacities. Enabled by this limiting assumption, \cite{geng_chance-constrained_2019} shows that the original scenario approach remains applicable in spite of the non-convexities from binary decision variables. Nonetheless, its main limitation is that the nice results in \cite{geng_chance-constrained_2019} only hold in the absence of transmission capacity constraints. This paper significantly improves \cite{geng_chance-constrained_2019} by considering additional security constraints such as line flow limits in the presence of uncertainties, and provides theoretical analysis on the results of the scenario approach.

The main contributions of this paper are threefold. (1) We contribute to the non-convex scenario approach theory by proving salient structural properties of non-convex scenario problems, which extends the classical results for convex scenario problems published in \cite{calafiore_random_2010}. (2) We formulate c-SCUC, which is later reformulated to scenario-based SCUC (s-SCUC) and solved via the scenario approach. To the best of our knowledge, this paper is the first to solve c-SCUC using the scenario approach while considering critical constraints such as transmission limits. (3) We design efficient algorithms to explore the structural properties of s-SCUC, which enables rigorous guarantees on the optimal solution returned by the scenario approach.

The remainder of this paper is organized as follows. Section \ref{sec:introduction_to_the_scenario_approach} summarizes the key results of the scenario approach for both convex and non-convex problems. Section \ref{sec:structural_properties_of_general_scenario_problems} proves the structural properties of non-convex scenario problems. Section \ref{sec:security_constrained_unit_commitment} formulates chance-constrained SCUC, which is solved via the scenario approach. Numerical results and discussions are in Section \ref{sec:case_study} and \ref{sec:discussions}, respectively. Section \ref{sec:concluding_remarks} presents the concluding remarks. All proofs are available in the full-length version \cite{geng_general_2019} of this paper.

The notations in this paper are standard.
All vectors are in the real field $\mathbf{R}$. We use $\mathbf{1}$ to represent an all-one vector of appropriate size. The transpose of a vector $a$ is $a^\intercal$.
The element-wise multiplication of the same-size vectors $a$ and $b$ is denoted by $a \circ b$. For instance, $[a_1;a_2] \circ [b_1;b_2] = [a_1 b_1; a_2 b_2]$.
Sets are in calligraphy fonts, e.g., $\mathcal{S}$. The cardinality of a set $\mathcal{S}$ is $|\mathcal{S}|$. Removal of element $i$ from set $\mathcal{N}$ is represented by $\mathcal{N}-i$. The essential supremum is $\esssup$.
% section introduction (end)

\section{Introduction to the Scenario Approach} % (fold)
\label{sec:introduction_to_the_scenario_approach}
This section first provides a brief introduction to chance-constrained optimization. Section \ref{sub:the_scenario_approach_for_convex_problems} presents the main results of the scenario approach for convex problems. Recent progress in the scenario approach for non-convex problems are summarized in Section \ref{sub:the_scenario_approach_for_non_convex_problems}.

\subsection{Chance-constrained Optimization} % (fold)
\label{sub:chance_constrained_optimization}
Chance-constrained optimization is a major approach for decision making in an uncertain environment.
Since its birth in 1950s \cite{charnes_cost_1958}, chance-constrained optimization has been widely studied and successfully applied in various fields \cite{geng_data-driven_2019-2}.
A typical formulation of chance-constrained optimization is presented below.
\begin{subequations}
\label{form:cc_opt_function}
\begin{align}
  \min_x~ &  c^\intercal x \\
 % & \text{s.t.} && \overline{Q_{CB}^{(i)}} = \frac{1}{T} \sum_{t=1}^{T} Q_{CB}^{(i)}[t]  & &  \\
  \text{s.t.}~&  \mathbb{P}_{\xi} \Big( f(x,\xi) \le 0 \Big) \ge 1 - \epsilon \label{form:cc_opt_function_cc} \\
  & g(x) \le 0 \label{form:cc_opt_function_det}
\end{align}
\end{subequations}
We could write \eqref{form:cc_opt_function} in a more compact form by defining $\mathcal{X}_\xi:= \{x \in \mathbf{R}^n: f(x,\xi) \le 0\}$ and $\chi := \{x \in \mathbf{R}^n: g(x) \le 0 \}$
\begin{subequations}
\label{form:cc_opt}
\begin{align}
  \min_{x \in \chi}~ &  c^\intercal x  \\
 % & \text{s.t.} && \overline{Q_{CB}^{(i)}} = \frac{1}{T} \sum_{t=1}^{T} Q_{CB}^{(i)}[t]  & &  \\
  \text{s.t.}~&  \mathbb{P}_{\xi} \Big( x \in \mathcal{X}_\xi \Big) \ge 1 - \epsilon \label{form:cc_opt_cc}
\end{align}
\end{subequations}
Without loss of generality, we assume that the objective is a linear function of decision variables $x \in \mathbf{R}^d$ \cite{campi_scenario_2009}. Random vector $\xi \in \Xi$ denotes the source of uncertainties and $\Xi$ is the support of $\xi$. Deterministic constraints \eqref{form:cc_opt_function_det} are represented by set $\chi$ in \eqref{form:cc_opt}. Constraint \eqref{form:cc_opt_function_cc} or \eqref{form:cc_opt_cc} is the \emph{chance constraint}. The chance constraint \eqref{form:cc_opt_cc} requires the the inner constraint $x \in \mathcal{X}_\xi$ to be satisfied with probability at least $1 - \epsilon$, where the violation probability $\epsilon$ is typically a small number (e.g., $1\%, 5\%$). In \eqref{form:cc_opt_cc}, the set $\mathcal{X}_\xi$ depends on the realization of $\xi$ and the probability is taken with respect to $\xi$.

Researchers have proposed many methods to solve chance-constrained optimization problems, e.g., sample average approximation \cite{pagnoncelli_sample_2009}, convex approximation \cite{nemirovski_convex_2006}, and scenario approach \cite{calafiore_uncertain_2005,campi_exact_2008,calafiore_random_2010}. A detailed review and tutorial on chance-constrained optimization is in \cite{geng_data-driven_2019-2}. Compared with other methods, the scenario approach has many advantages such as computationally efficient and are applicable for a broad range of optimization problems. 
% subsection chance_constrained_optimization (end)

\subsection{The Scenario Approach for Convex Problems} % (fold)
\label{sub:the_scenario_approach_for_convex_problems}
The scenario approach (sometimes referred as scenario approximation) is one of the well-known solutions to chance-constrained optimization, but its strength is not well-understood until recently \cite{geng_data-driven_2019-2}. 
The scenario approach utilizes $N$ independent and identically distributed (i.i.d.) scenarios $\mathcal{N} := \{\xi^1,\xi^2,\cdots,\xi^N\}$ to \FR{approximate} the chance-constrained program \eqref{form:cc_opt_function} with the \emph{scenario problem} below:
\begin{subequations}
\label{form:scenario_problem_function}
\begin{align}
  \text{SP}(\mathcal{N}):~\min_{x} \quad &  c^\intercal x  \\
 % & \text{s.t.} && \overline{Q_{CB}^{(i)}} = \frac{1}{T} \sum_{t=1}^{T} Q_{CB}^{(i)}[t]  & &  \\
  \text{s.t. } & f(x,\xi^1) \le 0 \label{form:scenario_problem_scenario_function_1}  & :\mu^{1} \\ 
  & \qquad \vdots \nonumber \\
  & f(x,\xi^N) \le 0 \label{form:scenario_problem_scenario_function_N}  & :\mu^{N}  \\
  & g(x) \le 0 &: \lambda
  \end{align}
\end{subequations}
The scenario problem $\SP(\N)$ seeks the optimal solution $x_{\mathcal{N}}^*$ that is feasible for all $N$ scenarios. The Lagrangian multiplier associated with the $i$th scenario constraint $f(x,\xi^{i}) \le 0$ is denoted by $\mu^{i} \in \mathbf{R}^m$. We can write the scenario problem $\SP(\N)$ in a similar way with \eqref{form:cc_opt} by defining $\mathcal{X}_{i}:= \{x \in \mathbf{R}^n: f(x, \xi^i) \le 0\}$.
\begin{subequations}
\label{form:scenario_problem_set}
\begin{align}
  \text{SP}(\mathcal{N}):~\min_{x \in \chi}~&  c^\intercal x  \\
 % & \text{s.t.} && \overline{Q_{CB}^{(i)}} = \frac{1}{T} \sum_{t=1}^{T} Q_{CB}^{(i)}[t]  & &  \\
  \text{s.t.}~&  x \in \cap_{i=1}^N \mathcal{X}_{i} \label{form:scenario_problem_scenario}
\end{align}
\end{subequations}
 \begin{defn}[Violation Probability]
The \emph{violation probability} of a candidate solution $x^\diamond$ is defined as the probability that $x^\diamond$ is infeasible:
\begin{equation}
\mathbb{V}(x^\diamond) := \mathbb{P}_\xi\big( x^\diamond \notin \mathcal{X}_\xi \big).
\end{equation}
\end{defn}
The scenario approach theory aims at answering the following \emph{sample complexity} question: what is the smallest sample size $N$ such that $x_{\mathcal{N}}^*$ is feasible (i.e., $\mathbb{V}(x_\mathcal{N}^*) \le \epsilon$) to the original chance-constrained program \eqref{form:cc_opt}? Reference \cite{campi_exact_2008,calafiore_random_2010} provide in-depth analysis based on the concept of support scenarios.
\begin{defn}[Support Scenario \cite{campi_exact_2008,calafiore_random_2010}]
\label{defn:support_scenario}
Scenario $\xi^i$ is a \emph{support scenario} for the scenario problem $\SP(\N)$ if its removal changes the solution of $\SP(\N)$.
\end{defn}
Let $x_{\N}^*$ and $x_{\N-i}^*$ stand for the optimal solution to scenario problems $\SP(\N)$ and $\SP(\N-i)$, respectively. Then scenario $\xi^i$ is a support scenario if $c^\intercal x_{\N-i}^* < c^\intercal x_{\N}^*$. We use $\Sc(\N)$ ($\Sc$ in short) to represent the set of all support scenarios of $\SP(\N)$.
\begin{defn}[Non-degenerate Scenario Problem \cite{campi_exact_2008,calafiore_random_2010}]
\label{defn:degenerate-convex}
Let $x_{\mathcal{N}}^*$ and $x_{\mathcal{S}}^*$ be the optimal solutions to the scenario problems $\SP(\N)$ and $\SP(\Sc)$, respectively. The scenario problem $\SP(\N)$ is said to be \emph{non-degenerate}, if $c^\intercal x_{\mathcal{N}}^* = c^\intercal x_{\mathcal{S}}^*$.
\end{defn}
\begin{assumption}[Non-degeneracy\cite{campi_exact_2008,calafiore_random_2010}]
\label{ass:non-degeneracy}
For every $N$, the scenario problem $\SP(\N)$ is non-degenerate with probability $1$ with respect to scenarios $\N = \{\xi^{1},\xi^{2},\cdots,\xi^{N}\}$.
\end{assumption}

\begin{assumption}[Feasibility \cite{campi_exact_2008}]
\label{ass:feasibility_uniqueness}
Every scenario problem $\SP(\N)$ is feasible, and its feasibility region has a non-empty interior. The optimal solution $x_{\mathcal{N}}^\ast$ of $\SP(\N)$ exists.
\end{assumption}
% The feasibility assumption can be further relaxed, more details can be found in \cite{calafiore_random_2010}.
\begin{defn}[Helly's Dimension \cite{calafiore_random_2010}]
Helly's dimension of the scenario problem $\SP(\N)$ is the least integer $h$ that 
$h \ge \esssup_{\N \subseteq \Xi^N} |\Sc(\N)|$ holds for any finite $N \ge 1$, where $|\Sc(\N)|$ is the number of support scenarios.
\end{defn}
Theorem \ref{thm:exact_feasibility_scenario_approach} presents one of the most important results in the scenario approach theory, which is based on the non-degeneracy and feasibility assumptions.
\begin{thm}[Exact Feasibility \cite{campi_exact_2008,calafiore_random_2010}]
\label{thm:exact_feasibility_scenario_approach}
Under Assumptions \ref{ass:non-degeneracy} (non-degeneracy) and \ref{ass:feasibility_uniqueness} (feasibility), let $x_{\N}^\ast$ be the optimal solution to the scenario problem $\SP(\N)$, it holds that
\begin{equation}
\label{eqn:exact_distribution_violation_prob}
  \mathbb{P}^N \Big( \mathbb{V}(x_{\N}^\ast)  > \epsilon \Big) \le \sum_{i=1}^{h-1} \binom{N}{i} \epsilon^i (1- \epsilon )^{N-i}.
\end{equation}
The probability $\mathbb{P}^N$ is taken with respect to $N$ random scenarios $\mathcal{N} = \{\xi^i\}_{i=1}^N$, and $h$ is the Helly's dimension of $\SP(\N)$.
\end{thm}
% The non-degeneracy assumption \ref{ass:non-degeneracy} lies at the heart of the scenario approach theory,
Stronger results without the feasibility assumption are in \cite{calafiore_random_2010,campi_exact_2008}.
Based on Theorem \ref{thm:exact_feasibility_scenario_approach}, the scenario approach answers the sample complexity question in Corollary \ref{cor:prior_sample_complexity_fully_supported}.
\begin{cor}[Sample Complexity \cite{campi_exact_2008,calafiore_random_2010}]
\label{cor:prior_sample_complexity_fully_supported}
Under Assumptions \ref{ass:non-degeneracy} (non-degeneracy) and \ref{ass:feasibility_uniqueness} (feasibility), given a violation probability $\epsilon \in (0,1)$ and a confidence parameter $\beta \in (0,1)$, if we choose the smallest number of scenarios $N$ such that 
\begin{equation}
  \sum_{i=0}^{h-1} \binom{N}{i} \epsilon^i (1- \epsilon)^{N-i} \le \beta,
\end{equation}
then it holds that
\begin{equation}
  \mathbb{P}^N\Big ( \mathbb{V}(x_{\mathcal{N}}^\ast) \le \epsilon \Big) \ge 1 - \beta,
\end{equation}  
where $x_{\mathcal{N}}^\ast$ is the optimal solution to $\SP(\N)$, and $h$ is the Helly's dimension of $\SP(\N)$ ($0 \le h \le N$). 
\end{cor}
The scenario approach is essentially a randomized algorithm to solve chance-constrained optimization problems. The randomness of the scenario approach comes from drawing i.i.d. scenarios. The confidence parameter $\beta$ quantifies the risk of failure due to drawing scenarios from a ``bad'' set. Corollary \ref{cor:prior_sample_complexity_fully_supported} shows that by choosing a proper number of scenarios, the corresponding optimal solution $x_{\mathcal{N}}^*$ is feasible (i.e., $\mathbb{V}(x_{\N}^*) \le \epsilon$) with confidence at least $1 - \beta$.
\begin{assumption}[Convexity]
\label{ass:convexity}
The deterministic constraint $g(x) \le 0$ is convex, and the random constraint $f(x,\xi)$ is convex in $x$ for every instance of $\xi$. In other words, the sets $\chi$ and $\mathcal{X}_i$s in \eqref{form:scenario_problem_set} are convex.
\end{assumption}
\begin{thm}[\cite{calafiore_uncertain_2005,calafiore_random_2010}]
\label{thm:helly_dimension_convex}
Under Assumption \ref{ass:feasibility_uniqueness} and \ref{ass:convexity}, 
the number of support scenarios $|\Sc|$ for $\SP(\N)$ is at most $n$. 
In other words, $h \le n$, where $n$ is the number of decision variables $x \in \mathbf{R}^n$ and $h$ is Helly's dimension. 
\end{thm}
For convex scenario problems $\SP(\N)$, we could replace $h$ by $n$ in Theorem \ref{thm:exact_feasibility_scenario_approach} and Corollary \ref{cor:prior_sample_complexity_fully_supported}. This leads to the classical results of the scenario approach in \cite{calafiore_uncertain_2005,campi_exact_2008,calafiore_random_2010}.
\begin{rem}[Towards Non-convexity]
Theorem \ref{thm:exact_feasibility_scenario_approach} and Corollary \ref{cor:prior_sample_complexity_fully_supported} do not assume convexity of $f(x,\xi)$ and $g(x)$. In theory, Theorem \ref{thm:exact_feasibility_scenario_approach} and Corollary \ref{cor:prior_sample_complexity_fully_supported} are applicable for non-convex scenario problems if a feasible non-convex $\SP(\N)$ is proved to be non-degenerate with probability $1$ (e.g., \cite{geng_chance-constrained_2019}). In practice, however, the scenario approach was considered \emph{not applicable} for non-convex problems. Comprehensive analysis are presented in Section \ref{sub:the_scenario_approach_for_non_convex_problems}.
\end{rem}
% subsection the_scenario_approach_for_convex_problems (end)

\subsection{The Scenario Approach for Non-convex Problems} % (fold)
\label{sub:the_scenario_approach_for_non_convex_problems}
The scenario approach was considered \emph{not applicable} for non-convex problems for the following three reasons: (1) non-convexity causes degeneracy; (2) non-trivial bounds on $|\Sc|$ may not exist for non-convex
$\SP(\N)$; and (3) it is computationally intractable to find optimal solutions.

First, degeneracy is a common issue for non-convex problems, e.g., the scenario-based SCUC problem in Section \ref{sub:s_scuc_is_degenerate}. 
Since the non-degeneracy assumption \ref{ass:non-degeneracy} lies at the heart of the scenario approach theory, almost all results in the literature are for non-degenerate problems.

Second, it is almost impossible to prove non-trivial and practical bounds on the number of support scenarios $|\Sc|$ for non-convex problems.
Reference \cite{campi_general_2018} presents one extreme case, in which every scenario is a support scenario thus $|\Sc|=N$ \footnote{Using the trivial bound $|\Sc| \le N$, Theorems \ref{thm:exact_feasibility_scenario_approach} and \ref{thm:scenario_theory_nonconvex_posterior} provide guarantees $\mathbb{P}( \mathbb{V}(x^*_{\N}) > \epsilon)\le 1$, which is useless.}. In addition, a loose bound typically leads to an astronomical sample complexity $N$, which make the scenario approach unpractical. For instance, loose bounds on $|\Sc|$ for scenario-based unit commitment will require $10^3 \sim 10^4$ times more scenarios than necessary \cite{geng_chance-constrained_2019}.

Furthermore, the most attractive feature of convex optimization is that any \emph{local} minimum is a \emph{global} minimum. And there exist a broad family of efficient algorithms that compute global optimal solutions for convex problems. Hence, $x_{\N}^*$ in Section \ref{sub:the_scenario_approach_for_convex_problems} refers to the \emph{global} optimal solution by default.
% Additionally, Theorem \ref{thm:helly_dimension_convex} stands on the fact that $x_{\N}^*$ is globally optimal.
It is worth noting that $x_{\N}^*$ is solely determined by the scenario problem $\SP(\N)$ and it is \emph{not} algorithm-dependent.

For non-convex problems, however, it is often computationally intractable to find global optimal solutions. There are many algorithms that are capable of finding \emph{local} optimal solutions in a relatively short time. Therefore, it is more reasonable and practical to analyze the characteristics of \emph{local} solutions for non-convex scenario problems. 
Algorithm  $\mathbb{A}: \Xi^N \rightarrow \mathbf{R}^n$ stands for the process of finding solutions to $\SP(\N)$, e.g., primal-dual interior-point method.
We use $\opx_\mathbb{A}(\N)$ to represent a (possibly suboptimal) solution to $\SP(\N)$ obtained via algorithm $\mathbb{A}$. The corresponding optimal objective value is denoted by $\opt_\mathbb{A}(\N)$. The subscript $\mathbb{A}$ emphasizes the fact that the solution is algorithm-dependent. And we use $\SP_\mathbb{A}(\N)$ to represent a scenario problem solved by algorithm $\mathbb{A}$.

Consequently, the scenario approach was considered \emph{not applicable} for non-convex problems until very recently. By removing the non-degeneracy assumption and analyzing any feasible solutions of non-convex scenario problems, reference \cite{campi_general_2018} develops a general theory for the scenario approach. This subsection summarizes its key results.

Identical to the convex case in Section \ref{sub:the_scenario_approach_for_convex_problems}, the scenario approach \FR{approximates} \eqref{form:cc_opt} to the scenario problem \eqref{form:scenario_problem_set} using $N$ scenarios $\mathcal{N} = \{\xi^1,\xi^2,\cdots, \xi^N\}$ for non-convex problems. The sets $\chi$ and $\mathcal{X}_\xi$ here could be non-convex.
% This procedure is depicted by algorithm $\mathbb{A}_N: \Xi^N \rightarrow \mathbf{R}^n$, which maps a set of scenarios $\N$ to a solution $\opx_\mathbb{A}(\N)$.
\begin{defn}[Invariant Set]
\label{def:invariant_set}
Let $\opt_\mathbb{A}(\mathcal{M})$ be the optimal value of $\SP(\mathcal{M})$ found by algorithm $\mathbb{A}$ for a scenario problem $\SP(\mathcal{M})$.
A set of scenarios $\mathcal{I}$ is an invariant (scenario) set for $\SP_\mathbb{A}(\N)$ if $\opt_\mathbb{A}(\mathcal{I}) = \opt_\mathbb{A}(\N)$.
\end{defn}
The concept of invariant set is an extension of support scenarios for (possibly degenerate) non-convex scenario problems. A trivial invariant set is $\Iv = \N$. Algorithm $\mathbb{B}: \Xi^N \rightarrow \Iv$ represents the process of finding non-trivial invariant sets. Examples of Algorithm $\mathbb{B}$ can be found in Section \ref{sec:structural_properties_of_general_scenario_problems} and Appendix \ref{sec:algorithms}.

\begin{thm}[Posterior Guarantees for Non-convex Scenario Problems \cite{campi_general_2018}\footnote{Theorem \ref{thm:scenario_theory_nonconvex_posterior} is a simplified version of the main result in \cite{campi_general_2018}, the feasibility assumption \ref{ass:feasibility_uniqueness} is a simplified version of the admissible assumption in \cite{campi_general_2018}.}]
\label{thm:scenario_theory_nonconvex_posterior}
Suppose Assumption \ref{ass:feasibility_uniqueness} (feasibility) holds true and $\beta \in (0,1)$ is given. Algorithm $\mathbb{A}$ solves the scenario problem $\SP(\N)$ and obtains an optimal solution $\opx_\mathbb{A}(\N)$. Algorithm $\mathbb{B}$ finds an invariant set $\mathcal{I}$ of cardinality $|\Iv|$. The following probabilistic guarantee holds
\begin{equation*}
  \mathbb{P}^N \Big( \mathbb{V}\big(\opx_\mathbb{A}(\N)\big) \le \epsilon(N,|\Iv|,\beta) \Big) \ge 1-\beta,
\end{equation*}
where the function $\epsilon(k,N,\beta)$ is defined as
\begin{equation}
\label{eqn:specified_epsilon_function}
\epsilon(N,k,\beta) := 
\begin{cases}
  1 & \text{if } k = N,\\
  1 - \Big( \frac{\beta}{ N \binom{N}{k}} \Big)^{\frac{1}{N-k}} & \text{otherwise.}
\end{cases}
\end{equation}
\end{thm}
\begin{lem}
\label{lem:monotonicity_specified_epsilon_function}
The $\epsilon(N,k,\beta)$ function defined in \eqref{eqn:specified_epsilon_function} has the following properties:
(1) $\epsilon(N,k,\beta)$ is monotonically decreasing in $\beta$;
(2) $\epsilon(N,k,\beta)$ is monotonically increasing in $k$;
(3) $\epsilon(N,k,\beta)$ is monotonically decreasing in $N$.
\end{lem}
In order to achieve an $\epsilon$-level solution with confidence $1-\beta$, Lemma \ref{lem:monotonicity_specified_epsilon_function} shows that the least conservative result (i.e., smallest sample complexity $N$) is achieved with the invariant set of minimal cardinality, which is defined as an essential set.
\begin{defn}[Essential Set \cite{calafiore_random_2010}]
\label{def:essential_set}
A set of scenarios $\Es \subseteq \N$ is an \emph{essential} (scenario) set for $\SP_\mathbb{A}(\N)$ if 
\begin{equation}
  \Es := \arg \min \{|\Es|: \opt_\mathbb{A}(\Es) = \opt_\mathbb{A}(\N), \Es \subseteq \N \}.
\end{equation}
In other words, $\Es$ is an invariant set of minimal cardinality.
\end{defn}
One key step in the non-convex scenario approach is designing algorithms $\mathbb{B}$ to search for essential sets. Section \ref{sec:structural_properties_of_general_scenario_problems} reveals the structure of general non-convex scenario problems, which lays the cornerstone for algorithms to obtain essential sets. Section \ref{sec:structural_properties_of_general_scenario_problems} also gives one example of designing more efficient algorithms by exploiting the structural properties of specific problems.
% subsection the_scenario_approach_for_non_convex_problems (end)
% section introduction_to_the_scenario_approach (end)

\section{Structural Properties of General Scenario Problems} % (fold)
\label{sec:structural_properties_of_general_scenario_problems}
Searching for essential sets is an important step in the non-convex scenario approach. However, the only known general algorithm to obtain essential sets is enumerating all $2^N$ possibilities by solving $2^N$ non-convex problems. This implies that searching for essential sets is in general computationally prohibitive. Section \ref{sub:non_convex_scenario_problems} first demonstrates the structural properties for general non-convex scenario problems, and proves a few special cases that finding essential sets is relatively easier. Section \ref{sub:convex_scenario_problems} reveals the connection between non-convex and convex scenario problems. Motivated by the structure of security-constrained unit commitment, Section \ref{sub:two_stage_scenario_problems} illustrates an efficient algorithm to track down essential sets for two-stage scenario problems.
\subsection{Non-convex Scenario Problems} % (fold)
\label{sub:non_convex_scenario_problems}
Instead of solving $2^N$ non-convex problems to obtain essential sets, there are two ideas to track down invariant sets with small cardinalities (not necessarily essential): (1) removing each scenario and checking if the objective changes, this idea leads to the definition of support sets; (2) removing scenarios one by one, until the scenario set cannot be further reduced, this leads to the definition of irreducible set.
\begin{defn}[Support Scenario of $\SP_{\mathbb{A}}(\N)$]
\label{defn:support_scenario_non_convex}
Scenario $\xi^i \in \N$ is a \emph{support scenario} for the scenario problem $\SP_\mathbb{A}(\N)$ if its removal changes the solution $\opt_\mathbb{A}(\N)$ of $\SP_\mathbb{A}(\N)$. The set of support scenarios (support set in short) is denoted by $\Sc_\mathbb{A}$. 
\end{defn}
\begin{defn}[Irreducible Set]
\label{def:irreducible_set}
A scenario set $\Ir \subseteq \N$ for $\SP_\mathbb{A}(\N)$ is \emph{irreducible}, if (1) it is invariant, i.e., $\opt_\mathbb{A}(\Ir) = \opt_\mathbb{A}(\N)$; and (2) $\opt_\mathbb{A}(\Ir-s) < \opt_\mathbb{A}(\Ir) = \opt_\mathbb{A}(\N)$ for any $s \in \Ir$.
\end{defn}
\begin{assumption}[Monotonicity]
\label{ass:monotone_algorithm}
Let $\mathbb{A}: \Xi^N \rightarrow \mathbf{R}^n$ be an algorithm to obtain the optimal solution of a scenario problem $\SP(\N)$, whose optimal objective value is represented by $\opt_\mathbb{A}(\N)$. We assume that the algorithm $\mathbb{A}$ always satisfies $\opt_\mathbb{A}(\mathcal{M}) \le \opt_\mathbb{A}(\N)$ if $\mathcal{M} \subseteq \N$.
\end{assumption}
Assumption \ref{ass:monotone_algorithm} is indeed a weak assumption. Considering two scenario problems $\SP(\N)$ and $\SP(\mathcal{M})$ with $\mathcal{M} \subseteq \N$. Because the optimal solution to $\SP(\N)$ will be always feasible to $\SP(\mathcal{M})$, algorithm $\mathbb{A}$ could use $\opx_\mathbb{A}(\N)$ as a starting point and obtain solution $\opx_\mathbb{A}(\mathcal{M})$ that is not worse than $\opx_\mathbb{A}(\N)$.
\begin{lem}[Modified Lemma 2.10 of \cite{calafiore_random_2010}]
\label{lem:support_is_subset_invariant_nonconvex}
Suppose algorithm $\mathbb{A}$ satisfies Assumption \ref{ass:monotone_algorithm}.
Let $\Iv$ be any \emph{invariant} set for a (possibly non-convex) scenario problem $\SP_\mathbb{A}(N)$ and $\Sc$ stands for its support set, then $\Sc \subseteq \Iv$. Since any essential set $\Es$ or irreducible set $\Ir$ is also invariant, then $\Sc \subseteq \Es$ and $\Sc \subseteq \Ir$.
\end{lem}
Lemma \ref{lem:support_is_subset_invariant_nonconvex} reveals the key relationship among the support set, essential and irreducible sets, and it lays the foundation of more important observations in Corollary \ref{cor:nondegenerate_uniqueness} and \ref{cor:nondegenerate_unique_essential_irreducible}.
Lemma \ref{lem:support_is_subset_invariant_nonconvex} is a generalized version of Lemma 2.10 in \cite{calafiore_random_2010}, which proved similar results for convex scenario problems. The importance of Lemma \ref{lem:support_is_subset_invariant_nonconvex} is to show that the key assumption for such structural properties is the monotonicity of algorithm $\mathbb{A}$, instead of convexity (Assumption \ref{ass:convexity} in \cite{calafiore_random_2010}).

For general (non-convex) scenario problems, the support set, essential set and irreducible set are different. Under certain circumstances, these three concepts are interchangeable. Such circumstances are depicted by an extended definition of non-degeneracy for non-convex scenario problems.
\begin{defn}[Non-degeneracy of $\SP_\mathbb{A}(\N)$]
\label{defn:degenerate-nonconvex}
For a general scenario problem $\SP_\mathbb{A}(\N)$, let $\N$ stand for the set of all $N$ scenarios and $\Sc$ denote the support (scenario) set. The scenario problem $\SP_{\mathbb{A}}(\N)$ is said to be \emph{non-degenerate}, if $\opt_\mathbb{A}(\N) = \opt_\mathbb{A}(\Sc)$.
\end{defn}
\begin{cor}
\label{cor:nondegenerate_uniqueness}
Consider a (possibly non-convex) scenario problem $\SP_\mathbb{A}(\N)$ and an algorithm $\mathbb{A}$ satisfying Assumption \ref{ass:monotone_algorithm}.  If $\SP_\mathbb{A}(\N)$ is non-degenerate, then (1) it has a unique essential set $\Es = \Sc$; and (2) it has a unique irreducible set $\mathcal{R} = \Sc$.
\end{cor}
\begin{cor}
\label{cor:nondegenerate_unique_essential_irreducible}
Consider a (possibly non-convex) scenario problem $\SP_\mathbb{A}(\N)$ and an algorithm $\mathbb{A}$ satisfying Assumption \ref{ass:monotone_algorithm}. The following three statements are equivalent with each other:
(1) $\SP_{\mathbb{A}}(\N)$ is non-degenerate;
(2) $\SP_{\mathbb{A}}(\N)$ has a unique irreducible set $\Ir$;
and (3) $\SP_{\mathbb{A}}(\N)$ has a unique essential set $\Es$.
\end{cor}
Corollaries \ref{cor:nondegenerate_uniqueness} and \ref{cor:nondegenerate_unique_essential_irreducible} provide key insights in designing an efficient algorithm $\mathbb{B}$. For non-convex problems, even if Assumption \ref{ass:non-degeneracy} does not always hold, $\SP_{\mathbb{A}}(\N)$ might be non-degenerate in many instances (e.g., s-SCUC is non-degenerate in 192 out of 200 instances in Section \ref{sub:finding_essential_sets_for_s_scuc}). For those non-degenerate scenario problems, Corollary \ref{cor:nondegenerate_uniqueness} and \ref{cor:nondegenerate_unique_essential_irreducible} show that we are able to find the essential set by solving only $N$ instead of $2^N$ non-convex problems. Section \ref{sub:two_stage_scenario_problems} shows that the computational burden to obtain essential sets can be further reduced by exploiting the structure of specific problems.
\begin{rem}[Finding Essential Sets for Non-degenerate Problems]
\label{rem:find_essential_sets_nondegenerate}
When a scenario problem is non-degenerate, we can obtain the (unique) essential set by searching for the support set or irreducible set (Corollary \ref{cor:nondegenerate_uniqueness}). 
Algorithms of finding an irreducible set (Algorithm \ref{alg:find-irreducible-set} in Appendix \ref{sec:algorithms}) or the support set (e.g., Algorithm \ref{alg:find-support-scenario-dual}) are based on definition. More discussions on finding the support set are in Remark \ref{rem:find_support_scenarios_convex}.
 % i.e., removing scenarios one by one until no single scenario can be further reduced.
% Remark \ref{rem:find_support_scenarios_convex} discusses the pursuit of support scenarios for  both convex and non-convex scenario problems.
\end{rem}

% subsection non_convex_scenario_problems (end)
\subsection{Convex Scenario Problems} % (fold)
\label{sub:convex_scenario_problems}
For convex scenario problems $\SP(\N)$, any local minimum is a global minimum. And a broad range of algorithms to look for global optimal solutions exist. In the convex setting, we assume any algorithm $\mathbb{A}$ returns global optimal solutions to $\SP(\N)$ by default. In Section \ref{sub:the_scenario_approach_for_convex_problems} and \ref{sub:convex_scenario_problems}, we replace $\opx_\mathbb{A}(\N)$ and $\opt_\mathbb{A}(\N)$ by $x_\mathcal{N}^*$ and $c^\intercal x_\mathcal{N}^*$, respectively. We also remove subscripts $\mathbb{A}$ since the definition of support set, invariant set and essential set for convex problems are no longer algorithm-dependent.
\begin{lem}[Monotonicity]
\label{lem:monotonicity}
Let $x_{\N}^*$ and $x_\mathcal{\mathcal{M}}^*$ stand for the global optimal solution to the (convex) scenario problems $\SP(\N)$ and $\SP(\mathcal{M})$, respectively. Then $c^\intercal x_{\mathcal{M}}^* \le c^\intercal x_{\N}^*$ if $\mathcal{M} \subseteq \mathcal{N}$. 
\end{lem}
Because $x_{\N}^*$ is always feasible to $\SP(\mathcal{M})$ and $x_{\mathcal{M}}^*$ is globally optimal, it is obvious that $c^\intercal x_{\mathcal{M}}^* \le c^\intercal x_{\N}^*$.
Lemma \ref{lem:monotonicity} shows that any algorithm obtaining global optimal solutions will automatically satisfy Assumption \ref{ass:monotone_algorithm}. Therefore, all results in Section \ref{sub:non_convex_scenario_problems} hold for convex scenario problems. It is worth mentioning that similar results for convex problems were first proved in \cite{calafiore_random_2010}. Section \ref{sub:non_convex_scenario_problems} can be regarded as an extension of classical results in \cite{calafiore_random_2010} towards non-convex scenario problems.
\begin{rem}[Finding Support Scenarios For Convex Problems]
\label{rem:find_support_scenarios_convex}
The first algorithm of searching for support scenarios (for both convex and non-convex scenario problems, Algorithm \ref{alg:find-support-set} in Appendix \ref{sec:algorithms}) is based on definition, i.e., checking if the removal of a scenario changes the optimal objective value.
Algorithm \ref{alg:find-support-set} requires solving $N$ scenario problems. In many cases (especially in power system applications, e.g., \cite{modarresi_scenario-based_2018}), it is observed that the support scenarios are only a small subset of all $N$ scenarios, i.e., $|\Sc| \ll |\N|$. This observation indicates the dual solution $\mu^1,\mu^2,\cdots,\mu^N$ to $\SP(\N)$ is often sparse.
Lemma \ref{lem:support_scenario_multiplier} formalizes this observation and provides an approach to narrow down the range of searching for support scenarios. Built upon Lemma \ref{lem:support_scenario_multiplier}, Algorithm \ref{alg:find-support-scenario-dual} only requires solving $\sim |\Sc|$ scenario problems, which is much more efficient than Algorithm \ref{alg:find-support-set} since $|\Sc| \ll |\N|$. 
\end{rem}

\begin{lem}
\FR{there should be a lemma about what the non-degenerate assumption implies}.
\end{lem}

\begin{thm}
\textcolor{blue}{Let $\mathcal{S}$ denote the set of support scenarios, and $\mathcal{M}$ is the set of scenarios with positive multipliers $\mathcal{M} := \{i \in \mathcal{N}: \|\mu^{i,*}\| > 0\}$. If $\SP(\N)$ is convex and non-degenerate, then $\mathcal{M} = \mathcal{S}$.}
\end{thm}
\begin{rem}
This is related with strict complementary slackness.
\end{rem}


\begin{lem}
\label{lem:support_scenario_multiplier}
Consider a non-degenerate and convex scenario problem $\SP(\N)$ which has at least one \emph{strictly} feasible solution. If $\xi^i$ is a support scenario ($i \in \Sc$), then $\|\mu^{i,*}\| > 0$, where $\mu^{i,*} \in \mathbf{R}^m$ is the optimal dual solution of $\SP(\N)$. In other words, let $\mathcal{M} := \{i \in \mathcal{N}: \|\mu^{i,*}\| > 0\}$, then $\Sc \subseteq \mathcal{M}$. \textcolor{blue}{(1) If $\xi^i$ is a support scenario ($i \in \Sc$), then $\|\mu^{i,*}\| > 0$; (2) If $\|\mu^{i,*}\| = 0$, then $\xi^i$ is not a support scenario ($i \notin \Sc$); (3) If $\xi^i$ is not a support scenario ($i \notin \Sc$), then $\|\mu^{i,*}\| = 0$; (4) If  $\|\mu^{i,*}\| > 0$, then $\xi^i$ is a support scenario ($i \in \Sc$). }
\end{lem}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE Compute the primal and dual solutions $x_{\mathcal{N}}^*$ and $\mu^{i,*}$ ($i=1,2,\cdots,N$) by solving $\SP(\N)$
\STATE Let $\mathcal{M} = \{i \in \mathcal{N}: \|\mu^{i,*}\| > 0\}$. Set $\mathcal{S} \leftarrow \emptyset$.
\FOR{$i \in \mathcal{M}$}
\STATE Solve $\text{SP}_{\mathcal{M}-i}$ and compute $x_{\mathcal{M}-i}^*$
\IF{$c^\intercal x_{\mathcal{M}-i}^* < c^\intercal x_{\mathcal{N}}^* (= c^\intercal x_{\mathcal{M}}^*)$} 
  \STATE $ \mathcal{S} \leftarrow \mathcal{S} + i$
\ENDIF
\ENDFOR
\end{algorithmic}
\caption{Finding Support Scenarios Using Dual Variables}
\label{alg:find-support-scenario-dual}
\end{algorithm}
In many cases, Algorithm \ref{alg:find-support-scenario-dual} only needs to solve the dual problem of $\SP(\N)$, it may not be necessary to solve the primal solution $x_{\N}^*$. We use $x_{\N}^*$ in Algorithm \ref{alg:find-support-scenario-dual} mainly for the purpose of notation simplicity.

\XG{show the simple constraint generation algorithm, and this works quite well for s-SCUC. Is bender decomposition related with things here?}.

A simple algorithm could do the job
 \FR{
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE Initialize $k=0$, $\mathcal{O} = \emptyset$, $\mathcal{M} = \emptyset$ and $\rho^* = +\infty$
\WHILE {$\rho^* \ge 0$}
\STATE Let $x^{(k)}$ be the optimal solution to 
\begin{subequations}
\begin{align}
x^{(k)} = \arg \min_{x}~& c^\intercal x \\
\text{s.t.}~& f_j(x, \xi^{i}) \le 0,~(i,j) \in \mathcal{O} \\
& g(x) \le 0
\end{align}
\end{subequations}
\STATE Find the scenario $i^*$ and constraint $j^*$ with the largest constraint violation $\rho^* = f_{j^*}(x, \xi^{i^*})$
\begin{equation}
\rho^* = \max_{j = \{1,2,\cdots,m.\}} \max_{i \in \mathcal{N}/\mathcal{M} } \big\{  f(x, \xi^{i}) \big\}
\end{equation}
\STATE $\mathcal{O} \leftarrow \mathcal{O} \cup \{(i^*, j^*)\}$, $\mathcal{M} \leftarrow \mathcal{M} \cup \{i^*\}$ and $k \leftarrow k+1$.
\ENDWHILE 
\STATE Output $x^{(k+1)}$, $\mathcal{M}$ and $\mathcal{O}$
\end{algorithmic}
\caption{ \FR{Solve Scenario Problem} }
\label{alg:solve-scenario-problem}
\end{algorithm}
}

\begin{rem}
Obviously Algorithm \ref{alg:solve-scenario-problem} converges in finite steps (worst case adding all $mN$ constraints). We observe that in xx, this algorithm converges in a much smaller number of iterations.
\end{rem}
% Algorithm \ref{alg:find-support-scenario-dual} is also utilized in finding essential sets for the non-convex two-stage scenario problems.
% subsection convex_scenario_problems (end)

\subsection{Two-stage Scenario Problems} % (fold)
\label{sub:two_stage_scenario_problems}
Section \ref{sub:non_convex_scenario_problems} shows that searching for essential sets can be relatively easier when a scenario problem is non-degenerate. However, finding a support set or irreducible set still requires solving $N$ non-convex problems. Motivated by SCUC, we show that more efficient algorithms are possible by exploiting the structure of specific problems. We study the following two-stage scenario problem in this subsection.
\begin{subequations}
\label{opt:two-stage-scenario-problem}
\begin{align}
\min_{y \in \mathcal{Y}}  c_y^\intercal y + \min_{\substack{x \in \mathcal{X}\\(x,y) \in \mathcal{H}}}~& c_x^\intercal x \\
\text{s.t.}~& x \in \cap_{i=1}^N \mathcal{U}_{i}
\end{align}
\end{subequations}
Constraints on the first-stage variables $y$ and the second-stage variables $x$ are denoted by $y \in \mathcal{Y}$ and $x \in \mathcal{X}$, respectively. Constraint $(x,y) \in \mathcal{H}$ represents the constraints coupling variables $x$ and $y$ in both stages. Set $\mathcal{U}_i$ stands for the constraints corresponding to the $i$th scenario $\xi^i$.

Problem \eqref{opt:two-stage-scenario-problem} is an abstract form of s-SCUC in Section \ref{sec:security_constrained_unit_commitment}.
Two key features of the two-stage scenario problem are: (1) the non-convexity \emph{only} comes from constraints $y \in \mathcal{Y}$ (e.g., binary variables in SCUC), all other constraints ($\mathcal{X}, \mathcal{H}, \mathcal{U}_i$) are convex; (2) uncertainties only exist in the second stage.

Let $(x^*, y^*)$ be a (possibly local) optimal solution that algorithm $\mathbb{A}$ returns. Given $y = y^*$, the second stage problem is convex by setting:
\begin{subequations}
\label{opt:second_stage_scenario_problem}
\begin{align}
\min_{\substack{x \in \mathcal{X}\\(x,y^*) \in \mathcal{H}}}~& c_x^\intercal x \\
\text{s.t.}~& x \in \cap_{i=1}^N \mathcal{U}_{i}
\end{align}
\end{subequations}
% WLOG, we assume that $x^*$ is the global optimal solution to the 2nd stage problem.
\begin{lem}
\label{lem:two_stage_support}
(1) Let $\hat{\Sc}$ represent the set of support scenarios of \eqref{opt:second_stage_scenario_problem} and $\Sc$ denote the support set for the two-stage problem \eqref{opt:two-stage-scenario-problem}, then $\hat{\Sc} \subseteq \Sc$; (2) If $\hat{\Sc}$ is invariant for \eqref{opt:two-stage-scenario-problem}, i.e., $\opt_\mathbb{A}(\hat{\Sc}) = \opt_\mathbb{A}(\N)$, then the two-stage scenario problem $\SP_{\mathbb{A}}(\N)$ is non-degenerate, \FR{and therefore $\mathcal{S} = \hat{\mathcal{S}}$. is it correct?}
\end{lem}
Corollaries \ref{cor:nondegenerate_uniqueness} and \ref{cor:nondegenerate_unique_essential_irreducible} demonstrate many nice properties of non-degenerate scenario problems.
Lemma \ref{lem:two_stage_support} gives a criteria of checking if the two-stage problem (e.g., s-SCUC) is non-degenerate. This lemma lays the foundation of Algorithm \ref{alg:find-support-subsample-structural} to search for essential sets of \eqref{opt:two-stage-scenario-problem}. The main idea of Algorithm \ref{alg:find-support-subsample-structural} is to first find the support scenarios of the second-stage problem \eqref{opt:second_stage_scenario_problem}, then verify if $\SP(\N)$ is degenerate using Lemma \ref{lem:two_stage_support}. In Section \ref{sub:finding_essential_sets_for_s_scuc}, it turns out that s-SCUC is non-degenerate in $96\%$ of cases, thus Algorithm \ref{alg:find-support-subsample-structural} could obtain essential sets of s-SCUC (in Section \ref{sub:finding_essential_sets_for_s_scuc}) in a much shorter time.

Generalized Benders Algorithm
% subsection two_stage_scenario_problems (end)
% section structural_properties_of_general_scenario_problems (end)

\section{Security-Constrained Unit Commitment with Probabilistic Guarantees} % (fold)
\label{sec:security_constrained_unit_commitment}
\subsection{Nomenclature} % (fold)
\label{sub:nomenclature}
The number of loads, generators, wind farms, transmission lines, contingencies, and snapshots are denoted by $n_d$, $n_g$, $n_w$, $n_l$, $n_k$ and $n_t$, respectively.
\begin{labeling}{$k \in \{0,1,\cdots,n_k\}$}
\item[$k \in \{0,1,\cdots,n_k\}$] contingency index
\item[$t \in \{0,1,\cdots,n_t\}$] time (snapshot) index
\item[$\iota \in \{t+1,\cdots,n_t\}$] additional time (snapshot) index in constraints \eqref{opt:det-SCUC-minon-time} and \eqref{opt:det-SCUC-minoff-time}
\end{labeling}
Binary decision variables (at time $t$):
\begin{labeling}{$z^{t} \in \{0,1\}^{n_g}$}
\item[$z^{t} \in \{0,1\}^{n_g}$] generator on/off states (commitment)
\item[$u^t \in \{0,1\}^{n_g}$] generator $i$ is on if $u_i^t = 1$
\item[$v^t \in \{0,1\}^{n_g}$] generator $i$ is off if $v_i^t = 1$ 
\end{labeling}
Continuous decision variables (at time $t$, contingency $k$):
\begin{labeling}{$g^{t,k} \in \mathbf{R}^{n_g}$}
\item[$g^{t,k} \in \mathbf{R}^{n_g}$] generation output
% $l^{t,k} \in \mathbf{R}^{n_d}$ & load shedding  \\
% $s^{t,k} \in \mathbf{R}^{n_d}$ & wind spillage/curtailment \\
\item[$r^{t} \in \mathbf{R}^{n_g}$] reserve 
\end{labeling}
Parameters and constants:
\begin{labeling}{$a^k \in \{0,1\}^{n_g}$}
% \item[$N^s, N^n$] Subset of buses with/without energy storage
\item[$a^k \in \{0,1\}^{n_g}$] generator availability in contingency $k$ 
\item[$\alpha_k \in \mathbf{R}_+$] weight of contingency $k$
\item[$c_g \in \mathbf{R}^{n_g}$] generation costs
\item[$c_z \in \mathbf{R}^{n_g}$] no load cost 
\item[$c_r \in \mathbf{R}^{n_g}$] reserve costs
\item[$c_u \in \mathbf{R}^{n_g}$] startup cost 
\item[$c_v \in \mathbf{R}^{n_g}$] shutdown cost 
\item[$\hat{d}^{t} \in \mathbf{R}^{n_d}$] load forecast (time $t$)
\item[$\tilde{d}^{t} \in \mathbf{R}^{n_d}$] load forecast error (time $t$)
\item[$\hat{w}^{t} \in \mathbf{R}^{n_w}$] wind forecast (time $t$) 
\item[$\tilde{w}^{t} \in \mathbf{R}^{n_w}$] wind forecast error (time $t$) 
\item[$\overline{g} \in \mathbf{R}^{n_g}$] generation upper bounds
\item[$\underline{g} \in \mathbf{R}^{n_g}$] generation lower bounds
\item[$\overline{\gamma} \in \mathbf{R}^{n_g}$] ramping upper bounds
\item[$\underline{\gamma} \in \mathbf{R}^{n_g}$] ramping lower bounds 
\item[$\underline{u}_i \in \mathbf{R}_+$] minimum on time for generator $i$
\item[$\underline{v}_i \in \mathbf{R}_+$] minimum off time for generator $i$
\end{labeling}

\subsection{Deterministic Security-constrained Unit Commitment} % (fold)
\label{sub:deterministic_unit_commitment}
Deterministic security-constrained unit commitment (d-SCUC) \eqref{opt:det-SCUC} seeks optimal commitment and startup/shutdown decisions $(z^t,u^t, v^t)$, generation and reserve schedules $(g^{t,k}, r^t)$ for a horizon of time steps, typically $24 \sim 36$ hours. The d-SCUC problem is being solved as a crucial part of the day-ahead market operation. Security constraints ensures the reliability of the power system after an unexpected event occurs.
\begin{subequations}
\label{opt:det-SCUC}
\begin{align}
\min_{z,u,v,g,r}~ & \sum_{t=1}^{n_t} \Big(  c_z^\intercal z^t + c_u^\intercal u^t + c_v^\intercal v^t + c_r^\intercal r^t + \sum_{k=0}^{n_k} \alpha_k c_g^\intercal g^{t,k} \Big) \label{opt:det-SCUC-obj} \\
\text{s.t.}~& \mathbf{1}^\intercal g^{t,k} + \mathbf{1}^\intercal \hat{w}^t  \ge \mathbf{1}^\intercal \hat{d}^t \label{opt:det-SCUC-balance}\\
& \underline{f} \le H_g^{t,k} g^{t,k} + H_w^{t,k} w^{t,k} - H_d^{t,k} d^{t,k} \le \overline{f} \label{opt:det-SCUC-line} \\
& a^k \circ \underline{\gamma} \le g^{t,k} - g^{t-1,k} \le a^k \circ \overline{\gamma}  \label{opt:det-SCUC-ramp} \\
& a^k \circ (g^{t,0} - r^t) \le g^{t,k} \le a^k \circ (g^{t,0} + r^t) \label{opt:det-SCUC-contingency} \\
% & a^k \circ  \underline{g} \circ  z^t \le g^{t,k} \le a^k \circ  \overline{g} \circ  z^t \label{opt:det-SCUC-contgencap-redundant} \\
& \hspace{109pt} k \in [0,n_k], t \in [1,n_t] \nonumber \\
& \underline{g} \circ  z^t \le g^{t,0} \le \overline{g} \circ  z^t \label{opt:det-SCUC-gencap}\\
& \underline{g} \circ  z^t \le g^{t,0} - r^t \le g^{t,0} + r^t \le \overline{g} \circ  z^t \label{opt:det-SCUC-resgencap}\\
& z^{t-1} - z^t + u^t \ge 0 \label{opt:det-SCUC-startup} \\
& z^t - z^{t-1} + v^t \ge 0 \label{opt:det-SCUC-shutdown} \\
& \hspace{157pt} t \in [1,n_t] \nonumber \\
& z_i^{t} - z_i^{t-1} \le z_i^\iota, ~ i \in [1,n_g] \label{opt:det-SCUC-minon-time} \\
& \hspace{23pt} \iota \in [t+1,\min\{t+\underline{u}_i-1,n_t\}], t \in [2,n_t] \nonumber \\
& z_i^{t-1} - z_i^{t} \le 1- z_i^\iota, ~ i \in [1,n_g] \label{opt:det-SCUC-minoff-time}\\
& \hspace{23pt} \iota \in [t+1,\min\{t+\underline{v}_i-1,n_t\}], t \in [2,n_t] \nonumber
\end{align}
\end{subequations}
The objective of \eqref{opt:det-SCUC} is to minimize total operation costs, including no-load costs $c_z^\intercal z^t$, startup costs $c_u^\intercal u^t$, shutdown costs $c_v^\intercal v^t$, generation costs $c_g^\intercal g^{t,k}$ and reserve costs $c_r^\intercal s^t$. Security constraints ensure: enough supply to meet demand \eqref{opt:det-SCUC-balance}, transmission line flow within limits \eqref{opt:det-SCUC-line}, generation levels within ramping limits \eqref{opt:det-SCUC-ramp} and capacity limits \eqref{opt:det-SCUC-gencap} in any contingency $k$. Constraints \eqref{opt:det-SCUC-contingency} and \eqref{opt:det-SCUC-resgencap} are about the relationship between generation and reserve in any contingency $k$. Constraints \eqref{opt:det-SCUC-startup}-\eqref{opt:det-SCUC-shutdown} are the logistic constraints about commitment status, startup and shutdown decisions. Minimum on/off time constraints for all generators are in \eqref{opt:det-SCUC-minon-time}-\eqref{opt:det-SCUC-minoff-time}. Constraints \eqref{opt:det-SCUC-ramp}-\eqref{opt:det-SCUC-resgencap} also guarantee the consistency of generation levels $g^{t,k}$ with commitment decisions $z^t$ and generator availability $a^k$ in contingency $k$ \cite{geng_chance-constrained_2019}. 
% subsection chance_constrained_scuc (end)

The d-SCUC formulation utilizes the expected wind generation and load forecast, it does not take the uncertainties from wind and load into consideration. We propose an improved formulation of d-SCUC using chance constraints, which explicitly guarantee the system security with a tunable level of risk $\epsilon$ with respect to uncertainties.
% \begin{subequations}
% \label{opt:c-SCUC-U}
% \begin{align}
% \mathbb{P}_{\tilde{w}\times\tilde{d}}\Big( \mathbf{1}^\intercal g^{t,k} + \mathbf{1}^\intercal (\hat{w}^t + \tilde{w}^t) \ge \mathbf{1}^\intercal (\hat{d}^t + \tilde{d}^t ), \label{opt:c-SCUC-balance-U} \\
% \underline{f} \le H_g^{t,k} g^{t,k} + H_w^{t,k} (\hat{w}^{t}+\tilde{w}^{t}) - H_d^{t,k} (\hat{d}^{t}+\tilde{d}^{t}) \le \overline{f}, \label{opt:c-SCUC-line-U} \\
% \hspace{1.5cm} k \in [0,n_k], t \in [1,n_t] \Big ) \ge 1 - \epsilon \nonumber
% \end{align}
% \end{subequations}
\begin{multline} \label{opt:c-SCUC-U}
\mathbb{P}_{\tilde{w}\times\tilde{d}}\Big( \mathbf{1}^\intercal g^{t,k} + \mathbf{1}^\intercal (\hat{w}^t + \tilde{w}^t) \ge \mathbf{1}^\intercal (\hat{d}^t + \tilde{d}^t ), \\
\underline{f} \le H_g^{t,k} g^{t,k} + H_w^{t,k} (\hat{w}^{t}+\tilde{w}^{t}) - H_d^{t,k} (\hat{d}^{t}+\tilde{d}^{t}) \le \overline{f}, \\
k \in [0,n_k], t \in [1,n_t] \Big ) \ge 1 - \epsilon
\end{multline}
\begin{subequations}
\label{opt:c-SCUC-U}
\begin{align}
 \nonumber
\end{align}
\end{subequations}
The formulation of chance-constrained Security-constrained Unit Commitment (c-SCUC) is presented below. Instead of using expected load $\hat{d}^t$ as in \eqref{opt:det-SCUC}, we consider loads $d^t$ as forecast $\hat{d}^t$ plus a random forecast error $\tilde{d}^t$ (i.e., $d^t = \hat{d}^t + \tilde{d}^t$).
\begin{align}
  \min~ &  \eqref{opt:det-SCUC-obj} \nonumber \\
\text{s.t.}~& \eqref{opt:det-SCUC-balance}\eqref{opt:det-SCUC-line}\eqref{opt:det-SCUC-ramp}\eqref{opt:det-SCUC-contingency}\eqref{opt:det-SCUC-gencap}\eqref{opt:det-SCUC-resgencap}\eqref{opt:det-SCUC-startup}\eqref{opt:det-SCUC-shutdown}\eqref{opt:det-SCUC-minon-time}\eqref{opt:det-SCUC-minoff-time} \nonumber \\
& \eqref{opt:c-SCUC-U} \nonumber 
\end{align}
Comparing with d-SCUC, the only difference of c-SCUC is the addition of the chance constraint \eqref{opt:c-SCUC-balance-U}. The chance constraint guarantees there will be enough supply to meet the net demand with probability no less than $1 - \epsilon$.

To reveal the structure of c-SCUC, we define the sets below:
\begin{subequations}
\begin{align}
\mathcal{B} &:= \big\{ (z,u,v): \eqref{opt:det-SCUC-startup}, \eqref{opt:det-SCUC-shutdown}, \eqref{opt:det-SCUC-minon-time}, \eqref{opt:det-SCUC-minoff-time} \big\}  \\
\mathcal{C} &:= \big\{ (g,r):  \eqref{opt:det-SCUC-balance}, \eqref{opt:det-SCUC-line}, \eqref{opt:det-SCUC-ramp}, \eqref{opt:det-SCUC-contingency} \big\}  \\
\mathcal{H} &:= \big\{ (z,g,r): \eqref{opt:det-SCUC-gencap}, \eqref{opt:det-SCUC-resgencap}  \big\} \\
\mathcal{U} &:= \big\{(g): \eqref{opt:c-SCUC-U}  \big\} 
\end{align}
\end{subequations}
Then c-SCUC can be succinctly represented as:
\begin{align*}
\min_{z,u,v,g,r}~ & \eqref{opt:det-SCUC-obj}  \\
\text{s.t.}~ &  (z,u,v) \in \mathcal{B} \\
& (g,r) \in \mathcal{C},~(z,g,r) \in \mathcal{H}\\
& \mathbb{P}\big ( g \in \mathcal{U}  \big) \ge 1 - \epsilon
\end{align*}
Sets $\mathcal{B}$ and $\mathcal{C}$ stand for the \emph{deterministic} constraints for binary and continuous variables, respectively. 
Set $\mathcal{H}$ represents the hybrid constraints related with both continuous and binary variables. Set $\mathcal{U}$ denotes all constraints related with uncertainties.
Using the scenario approach, c-SCUC is \FR{approximated by} the scenario-based SCUC (s-SCUC) problem below:
\begin{align*}
\min_{(z,u,v) \in \mathcal{B}}~& \sum_{t=1}^{n_t} \Big( c_z^\intercal z^t + c_u^\intercal u^t + c_v^\intercal v^t \Big) + \\
& \min_{(z,g,r) \in \mathcal{H}} \sum_{t=1}^{n_t} \Big( c_r^\intercal r^t + \sum_{k=0}^{n_k} \alpha_k c_g^\intercal g^{t,k} \Big) \nonumber \\
 & \hspace{1cm}\text{s.t.}~ (g,r) \in \mathcal{C} \\
 & \hspace{1.5cm} g \in \cap_{i=1}^N \mathcal{U}_i \nonumber 
\end{align*}
\begin{rem}[Structural Properties of SCUC]
\label{rem:structural_prop_c-SCUC}
SCUC is a two-stage optimization problem by nature, it has the following nice properties. Firstly, the non-convexity \emph{only} exists in the first stage, i.e., $y \in \mathcal{Y}$. Given a first-stage solution $y$, the second stage is a simple linear program. Secondly, uncertainties come from renewables in the operation stage (only in the second stage).
% The abstract form \eqref{opt:two-stage-scenario-problem} of of s-SCUC highlights these two .
Based on the nice structural properties above, Section \ref{sub:two_stage_scenario_problems} shows that we are able to track down essential sets by solving two MILPs and $\sim |\Sc|$ linear programs.
\end{rem}

\subsection{Degeneracy of s-SCUC} % (fold)
\label{sub:s_scuc_is_degenerate}
This section presents an example to show that s-SCUC could be degenerate in many cases, which violates Assumption \ref{ass:non-degeneracy}. Therefore almost all results of the classical scenario approach are not applicable. For s-SCUC, theoretical guarantees are only possible through the non-convex scenario approach in Section \ref{sub:the_scenario_approach_for_non_convex_problems}.

We use a 3-bus system to illustrate the degeneracy of s-SCUC. Configurations of the 3-bus system are in \cite{geng_general_2019}. In order to visualize the feasible region of s-SCUC, we simplify the problem by (1) only considering one snapshot ($n_t=1$) and ignoring initial status (thus no $u,v$ variables); (2) removing reserve constraints (no $r$ variables). By doing this, there are only four decision variables left: $z_1, z_2, g_1,g_2$. The on/off states $z_1,z_2$ can be inferred from values of $g_1$ and $g_2$, therefore the feasible region of the simplified s-SCUC can be visualized on the $(g_1, g_2)$-plane.

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=\linewidth]{case3-degenerate-example-all.pdf}
% 	\caption{An illustrative example that s-SCUC is degenerate (3-bus system), illustration of the feasible region with constraints of all scenarios ($\mathcal{U}_1$,$\mathcal{U}_2$,$\mathcal{U}_3$).}
% 	\label{fig:case3-degenerate-example-all}
% \end{figure}

% \begin{figure}[htbp]
% 	\centering
% 	\includegraphics[width=\linewidth]{case3-degenerate-example-support.pdf}
% 	\caption{An illustrative example that s-SCUC is degenerate (3-bus system), illustration of the feasible region with only support scenarios ($\mathcal{U}_1$).}
% 	\label{fig:case3-degenerate-example-support}
% \end{figure}

\begin{figure*}[htbp]
  \centering
  \subfloat[Illustration of the feasible region with constraints of all scenarios ($\mathcal{U}_1$,$\mathcal{U}_2$,$\mathcal{U}_3$).]{\includegraphics[width=0.5\linewidth]{case3-degenerate-example-all.pdf}\label{fig:case3-degenerate-example-all}} 
  \subfloat[Illustration of the feasible region with only support scenarios ($\mathcal{U}_1$).]{\includegraphics[width=0.5\linewidth]{case3-degenerate-example-support.pdf}\label{fig:case3-degenerate-example-support}} 
  \caption{An illustrative example that s-SCUC is degenerate (3-bus system)}
  \label{fig:case3-degenerate-example}
\end{figure*}

Using Definition \ref{defn:degenerate-convex}, showing the degeneracy of s-SCUC includes three steps: (1) obtaining the optimal solution to $\SP(\N)$; (2) finding all support scenarios $\Sc$ of $\SP(\N)$; and (3) checking if the optimal solution of $\SP(\N)$ is the same as $\SP(\Sc)$.
Fig. \ref{fig:case3-degenerate-example-all} first visualizes constraints $\mathcal{B}_0\sim \mathcal{B}_3$, which represents the region of 4 possible generator on/off status (e.g., $\mathcal{B}_1: z_1=1, z_2 =0$, $\mathcal{B}_3: z_1=1, z_2 =1$). The black solid lines denote constraints \eqref{opt:det-SCUC-balance}, \eqref{opt:det-SCUC-line} and \eqref{opt:det-SCUC-gencap} using forecast values (d-SCUC). The red, yellow and purple dotted lines are three sets ($\mathcal{U}_1,\mathcal{U}_2,\mathcal{U}_3$) of constraints corresponding to three scenarios.
Given the setting that generator 1 is much cheaper than generator 2, we can easily eyeball the optimal solution with all constraints presented, marked by the red $*$. Next, we observe that removing scenario 1 ($\mathcal{U}_1$, red lines) changes the optimal solution, while removing scenario scenario 2 ($\mathcal{U}_2$, yellow lines) or scenario 3 ($\mathcal{U}_3$, purple lines) makes no difference. Thus scenario 1 is the only support scenario. Finally, we examine the scenario problem with only support scenarios presented. Fig. \ref{fig:case3-degenerate-example-support} shows that the optimal solution becomes the red $\diamond$ with only scenario 1, which is clearly different than the optimal solution in Fig. \ref{fig:case3-degenerate-example-all}. Hence, s-SCUC is a degenerate problem.


\subsection{Decomposition Algorithm for s-SCUC} % (fold)
\label{sub:decomposition_algorithm_for_s_scuc}

% subsection decomposition_algorithm_for_s_scuc (end)

% subsection s_scuc_is_degenerate (end)
% section security_constrained_unit_commitment (end)

\section{Case Study} % (fold)
\label{sec:case_study}
\subsection{Settings of the 118-bus System} % (fold)
Numerical simulations were conducted on a modified 118-bus, 184-line, 54-generator, 24-hour system \cite{illinois_institute_of_technology_ieee_2004}. Most settings are identical as \cite{illinois_institute_of_technology_ieee_2004}, except 5 wind farms are added to the system as in \cite{pena_extended_2018}. The s-SCUC problems were solved using $64$ GB memory on the Hera server (hera.ece.tamu.edu), provided by Texas A\&M University. The mathematical models for s-SCUC was formulated using YALMIP \cite{lofberg_yalmip_2004} on Matlab R2019a and solved using Gurobi v8.1 \cite{gurobi_optimization_gurobi_2016}.

After obtaining a solution $\opx_{\mathbb{A}}(\N)$ to s-SCUC, Theorem \ref{thm:scenario_theory_nonconvex_posterior} provides an upper bound $\epsilon(N,|\Iv|,\beta)$ on the \emph{actual} violation probability $\mathbb{V}(\opx_{\mathbb{A}}(\N))$. The theoretical guarantee $\epsilon(N,|\Iv|,\beta)$ is referred as posterior $\epsilon$ in the numerical results. The actual violation probability $\mathbb{V}(\opx_{\mathbb{A}}(\N))$ is estimated by the out-of-sample violation probability $\hat{\epsilon}$, using an independent set of $10^6$ scenarios.

To quantify the randomness of the scenario approach, for each sample complexity $N=100,200,\cdots,1000$, we solve the corresponding s-SCUC problems on 10 independent sets of scenarios (i.e., $10$ Monte-Carlo simulations). Results in both Fig. \ref{fig:sc-SCUC-case118iit-fig_obj0eps0_2axis} and \ref{fig:sc-SCUC-case118iit-epsilon-epsilon} show the average, maximum and minimum values in 10 Monte-Carlo simulations. 

% We mainly examine the quality of solution to s-SCUC in the following aspects: (1) economic efficiency, quantified by the total operation cost; (2) system security, quantified by the out-of-sample violation probability $\hat{\epsilon}$, evaluated on an independent set of $10^6$ scenarios; and (3) structural properties, mainly the cardinality of essential sets.

% subsubsection settings (end)
\subsection{Cost vs Security: a trade-off} % (fold)
\label{ssub:cost_security_trade_off}
Fig. \ref{fig:sc-SCUC-case118iit-fig_obj0eps0_2axis} shows the out-of-sample violation probability $\hat{\epsilon}$ and objective value (total cost). The shadowed area shows the max-min values in 10 Monte-Carlo simulations, and the solid line is the average value of 10 independent simulations. It is shown that the system risk level (violation probability) is reduced by $83\%$ (from $\sim 30\%$ to $\sim 5\%$) by $\sim1.1\%$ increase in total system costs. Similar observations were found in \cite{modarresi_scenario-based_2018,geng_data-driven_2019-2,geng_chance-constrained_2019}.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{sc-SCUC-case118iit-fig_obj0eps0_2axis.pdf}
  \caption{Cost vs Security: a Trade-off.}
  \label{fig:sc-SCUC-case118iit-fig_obj0eps0_2axis}
\end{figure}

% subsubsection cost_security_trade_off (end)

\subsection{Violation Probability} % (fold)
\label{ssub:violation_probability}
Fig. \ref{fig:sc-SCUC-case118iit-epsilon-epsilon} presents the out-of-sample violation probability $\hat{\epsilon}$ and theoretical guarantees (posterior $\epsilon$ provided by Theorem \ref{thm:scenario_theory_nonconvex_posterior}). Since the cardinality of essential sets differ for each scenario problem (Fig. \ref{fig:sc-SCUC-case118iit-support-scenario-number}), the posterior guarantee $\epsilon$ is a band instead of a line. As illustrated in Fig. \ref{fig:sc-SCUC-case118iit-epsilon-epsilon}, the actual violation probability (approximated by $\hat{\epsilon}$) is bounded by the theoretical guarantees. This verifies the correctness of Theorem \ref{thm:scenario_theory_nonconvex_posterior}. The conservative ratio is $2\sim 4$ (e.g., when out-of-sample $\hat{\epsilon}$ is $\sim5\%$, Theorem \ref{thm:scenario_theory_nonconvex_posterior} gives an upper bound $10\% \sim 20\%$).
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{sc-SCUC-case118iit-epsilon-epsilon.pdf}
  \caption{Out-of-sample Violation Probabilities and Theoretical Guarantees.}
  \label{fig:sc-SCUC-case118iit-epsilon-epsilon}
\end{figure}
% subsubsection violation_probability (end)

\subsection{Searching for Essential Sets for s-SCUC} % (fold)
\label{sub:finding_essential_sets_for_s_scuc}
s-SCUC was observed to be non-degenerate in 192 out of 200 simulations\footnote{We conducted 10 simulation for 10 different sample complexities ($100,200,\cdots,1000$) under two different settings: with/without $N-1$ contingencies, both include transmission constraints.}. In other words, in $96\%$ cases, we are able to find an essential set by solving $5\sim35$ linear programs and $2$ mixed integer linear programs. 
It takes from 4934 seconds ($N=100$) to 6847 seconds ($N=1000$) to solve one MILP (s-SCUC). When searching for support scenarios for the second-stage problem (a linear program), it takes $281 \sim 388$ seconds to solve one LP.
For those 8 out of 200 simulations, it takes an extra $20$ hours to find an irreducible set using Algorithm \ref{alg:find-irreducible-set}. This computation time can be greatly reduced by tricks such as choosing appropriate starting points\footnote{For example, when removing scenarios $s$ and $t$ consecutively in Algorithm \ref{alg:find-irreducible-set}, the solution $\opt_\mathbb{A}(\N-s)$ is feasible to $\SP(\N-s-t)$ thus can serve as a good starting point.}.
% subsection finding_essential_sets_for_s_scuc (end)

% section case_study (end)

\section{Discussions} % (fold)
\label{sec:discussions}

\subsection{Cardinality of Essential Sets} % (fold)
\label{sub:cardinality_of_essential_sets}
Fig. \ref{fig:sc-SCUC-case118iit-support-scenario-number} compares the cardinalities of essential sets for three cases: (a) c-SCUC with $N-1$ contingencies but without transmission constraints, results of case (a) are obtained from \cite{geng_chance-constrained_2019}); (b) c-SCUC with transmission constraints but without $N-1$ contingencies; and (c) c-SCUC with both transmission constraints and $N-1$ contingencies.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{sc-SCUC-case118iit-support-scenario-number.pdf}
  \caption{Cardinality of Essential Sets. \XG{Y-axis to be fixed}}
  \label{fig:sc-SCUC-case118iit-support-scenario-number}
\end{figure}

Case (a) is the simplest, in \cite{geng_chance-constrained_2019} we show that the scenario problem for unit commitment satisfies the non-degeneracy assumption \ref{ass:non-degeneracy}, and the cardinality of essential sets is bounded by the number of snapshots $n_t$, i.e., $|\Sc| \le n_t = 24$ in Fig. \ref{fig:sc-SCUC-case118iit-support-scenario-number}. Cases (b) and (c) include transmission capacity constraints. As demonstrated in Section \ref{sub:s_scuc_is_degenerate}, s-SCUC could be degenerate with transmission constraints. Theoretically speaking, the cardinality of essential sets might be unbounded for non-convex problems. \FR{Fig. \ref{fig:sc-SCUC-case118iit-support-scenario-number} shows that the cardinality of essential sets is greatly smaller than the number of decision variables. For example, s-SCUC has about $4000$ binary variables and around $75000$ continuous decision variables, while the cardinalities of essential sets are $30\sim40$ in case (b) and $0\sim10$ in case (c).} This observation implies that the number of scenarios $N$ required could be much smaller than expected. 

Another interesting observation is that including $N-1$ contingency constraints reduces $|\Es|$. This observation has two implications. First, $N-1$ contingency constraints not only protect the system from unexpected device failures, they also help reduce the impacts of uncertainties from renewables. Second, including $N-1$ contingency constraints could help reduce sample complexity. Similar with the observations in \cite{modarresi_scenario-based_2018}, this observation indicates that the scenario approach might be of practical use.

\subsection{From Posterior to Prior Guarantees} % (fold)
\label{sub:from_posterior_to_prior_guarantees}
Theorem \ref{thm:scenario_theory_nonconvex_posterior} gives \emph{posterior} guarantees on the quality of solutions, namely, we calculate $\epsilon(N,k,\beta)$ \emph{after} obtaining the solution $\opx(\N)$.  
Lemma \ref{lem:monotonicity_specified_epsilon_function} proves that the $\epsilon(N,k,\beta)$ function in \eqref{eqn:specified_epsilon_function} is monotone in $N$ and $k$. This implies that we can obtain prior guarantees. In other words, if the cardinality of essential sets is proved to be at most $h$ ($|\Es| \le h$), then we can find the smallest $\hat{N}$ such that
\begin{equation}
\epsilon \ge 1 - \Big( \frac{\beta}{ \hat{N} \binom{\hat{N}}{h}} \Big)^{\frac{1}{\hat{N}-h}}
\end{equation}
holds for given $\epsilon$ and $\beta$. Then the solution $\opx_{\mathbb{A}}(\N)$ to the scenario problem using $\hat{N}$ scenarios has the guarantee $\mathbb{P}(\mathbb{V}(\opx_{\mathbb{A}}(\N)) \le \epsilon) \ge 1 - \beta$. This prior guarantee holds \emph{before} solving the scenario problem with $\hat{N}$ scenarios. If a rigorous bound $h$ on $|\Es|$ can be proved, then there is no need to numerically search for essential sets. This is particularly attractive compared with posterior guarantees.
% subsection from_posterior_to_prior_guarantees (end)
% section discussions (end)

\section{Concluding Remarks} % (fold)
\label{sec:concluding_remarks}
This paper solves chance-constrained SCUC via the scenario approach and obtains rigorous theoretical guarantees on the solution. We demonstrate the structural properties of (possibly non-convex) general scenario problems. To obtain the tightest theoretical guarantees for chance-constrained SCUC, we design efficient algorithms to search for essential sets by exploiting the salient structures of SCUC.
Numerical results on an IEEE benchmark system show that the essential scenario set is only a small subset of all scenarios. This implies that we can obtain relatively robust solutions (i.e., small $\epsilon$) using only a moderate number of scenarios. Furthermore, we observe that some power engineering practices (e.g., $N-1$ criteria) can help us reduce the number of scenarios needed while maintaining the same level of risk.

Future work includes reducing conservativeness by improving the complexity bound in Theorem \ref{thm:scenario_theory_nonconvex_posterior} and investigating the performance of the (non-convex) scenario approach on larger-scale realistic systems.
% section concluding_remarks (end)
